Multimodal Transformer for Unaligned Multimodal Language Sequences

Human language is often multimodal, which comprehends a mixture of natural language, facial gestures, and acoustic behaviors. However, two major challenges in modeling such multimodal human language time-series data exist: 1) inherent data non-alignment due to variable sampling rates for the sequences from each modality; and 2) long-range dependencies between elements across modalities. In this paper, we introduce the Multimodal Transformer (MulT) to generically address the above issues in an end-to-end manner without explicitly aligning the data. At the heart of our model is the directional pairwise crossmodal attention, which attends to interactions between multimodal sequences across distinct time steps and latently adapt streams from one modality to another. Comprehensive experiments on both aligned and non-aligned multimodal time-series show that our model outperforms state-of-the-art methods by a large margin. In addition, empirical analysis suggests that correlated crossmodal signals are able to be captured by the proposed crossmodal attention mechanism in MulT.

==> tables/asynchornous.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\begin{table}[t!]
\caption{\small Results for multimodal sentiment analysis on CMU-MOSEI with asynchronous multimodal sequences. Crossmodal transformer outperforms recent SOTA models on both aligned and non-aligned sequences.}
\begin{center}
\fontsize{7}{10}\selectfont
%\centering
\setlength\tabcolsep{0.7pt}
\vspace{-2mm}
\begin{tabular}{|c||*{5}{K{0.77cm}}|}
\hline
Metric         & Acc$_7^h$  & Acc$_2^h$  & F1$^h$    & MAE$^l$   & Corr$^h$  \\ \hline \hline
\multicolumn{6}{|c|}{(Word Aligned But Asynchronous) CMU-MOSEI Sentiment}     \\ \hline \hline
EF-LSTM        & 43.0  & 73.2  & 72.5  & 0.74 & 0.47 \\
LF-LSTM        & 48.8    & 80.6  & 80.6  & 0.619 & 0.659 \\
MCTN~\cite{pham2018found}           & 49.6     & 79.8  & 80.6  & 0.609 & 0.670 \\
RAVEN~\cite{wang2018words}          & 50.0     & 79.1  & 79.5     & 0.614 & 0.662 \\ \hline \hline
Ours           & \bf{51.8}     & \bf{82.4}  & \bf{82.2}  & \bf{0.580} & \bf{0.703} \\ \hline \hline
\multicolumn{6}{|c|}{(Non-Aligned) CMU-MOSEI Sentiment} \\ \hline \hline
CTC~\citep{graves2006connectionist} + EF-LSTM  & 44.8     & 69.7  & 69.5  & 0.755 & 0.401 \\
LF-LSTM        & 49.9     & 80.0  & 80.2  & 0.620 & 0.650 \\
CTC + MCTN~\cite{pham2018found}     & 46.9     & 80.2  & 80.6  & 0.611 & 0.664 \\
CTC + RAVEN~\cite{wang2018words}    & 48.9     & 76.2  & 77.0  & 0.681 & 0.576 \\ \hline \hline
Ours           & \textbf{51.6}   & \textbf{81.8}  & \textbf{81.7}  & \textbf{0.586} & \textbf{0.697} \\ \hline
\end{tabular}
\end{center}
\end{table}

==> tables/shift_iemocap.tex <==




\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\begin{table*}[t!]
\vspace{-5mm}
\caption{\small Results for multimodal emotions analysis on IEMOCAP with aligned and non-aligned multimodal sequences.}
\begin{center}
\fontsize{7}{10}\selectfont
%\centering
\setlength\tabcolsep{0.7pt}
\vspace{-2mm}
\begin{tabular}{|c||*{8}{K{0.8cm}}|}
\hline
Task          & \multicolumn{2}{c}{Happy} & \multicolumn{2}{c}{Sad} & \multicolumn{2}{c}{Angry} & \multicolumn{2}{c|}{Neutral} \\
Metric        & Acc$^h$         & F1$^h$          & Acc$^h$        & F1$^h$         & Acc$^h$         & F1$^h$          & Acc$^h$           & F1$^h$           \\ \hline \hline
\multicolumn{9}{|c|}{(Shifted) IEMOCAP Emotions}                                                                           \\ \hline  \hline
EF-LSTM  &   &   &   & \multicolumn{2}{c}{Does not converge}  &   &   &  \\
LF-LSTM       & 86.0  & 84.1  &  81.6 & 80.9 &  87.1 &  86.6 & 68.4 & 68.6         \\
MCTN~\cite{pham2018found}   &   &   &   & \multicolumn{2}{c}{Does not converge}  &   &   &  \\
RAVEN~\cite{wang2018words}   &   &   &   & \multicolumn{2}{c}{Does not converge}  &   &   &  \\  \hline \hline
Ours          & -  & -  &  - & - &  - &  - & - & -        \\ \hline  
%\hline \multicolumn{9}{|c|}{(Old Non-Aligned) IEMOCAP Emotions}                                                                           \\ \hline  \hline
% CTC~\cite{graves2006connectionist} + EF-LSTM & 85.6$^*$           & n/a           & 78.8          & 70.2          & 75.8$^*$           & n/a          & 59.2$^*$           & n/a            \\
%CTC~\cite{graves2006connectionist} + EF-LSTM  &   &   &   & \multicolumn{2}{c}{Does not converge}  &   &   &   \\
%LF-LSTM       & 80.2        & 78.3        & 79.4$^*$       & n/a       & 70.4        & 69.1        & 56.7          & 56.0         \\
% CTC + MCTN~\cite{pham2018found}    & 85.6$^*$           & n/a          & 79.4$^*$          & n/a          & 75.8$^*$           & n/a           & 59.2$^*$             & n/a            \\
%CTC + MCTN~\cite{pham2018found}   &   &   &   & \multicolumn{2}{c}{Does not converge}  &   &   &   \\
% CTC + RAVEN~\cite{wang2018words}   & 85.6$^*$           & n/a           & 79.4$^*$      & n/a          & 75.8$^*$           & n/a           & 59.2$^*$            & n/a            \\ \hline  \hline
%CTC + RAVEN~\cite{wang2018words}  &   &   &   & \multicolumn{2}{c}{Does not converge}  &   &   &   \\  \hline \hline
%Ours          & \bf{87.8}        & \bf{83.5}        & \bf{80.0}       & \bf{71.9}       & \bf{76.6}        & \bf{72.2}        & \bf{61.0}          & \bf{58.4}         \\ \hline
\end{tabular}
\end{center}
\vspace{-5mm}
\end{table*}

==> tables/shift_mosei.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\begin{table}[t!]
\caption{\small Results for multimodal sentiment analysis on (relatively large scale) CMU-MOSEI with aligned and non-aligned multimodal sequences. Crossmodal transformer outperforms recent SOTA models on both aligned and non-aligned sequences.}
\begin{center}
\fontsize{7}{10}\selectfont
%\centering
\setlength\tabcolsep{0.7pt}
\vspace{-2mm}
\begin{tabular}{|c||*{5}{K{0.77cm}}|}
\hline
Metric         & Acc$_7^h$  & Acc$_2^h$  & F1$^h$    & MAE$^l$   & Corr$^h$  \\ \hline \hline
\multicolumn{6}{|c|}{(Shifted) CMU-MOSEI Sentiment} \\ \hline \hline
EF-LSTM  & 44.5     & 71.8  & 71.7  & 0.753 & 0.418 \\
LF-LSTM        & 49.6     & 76.8  & 76.9  & 0.612 & 0.654 \\
MCTN~\cite{pham2018found}     & 49.1     & 79.3  & 80.0  & 0.617 & 0.652 \\
RAVEN~\cite{wang2018words}    & 47.6     & 78.2  & 78.0  & 0.645 & 0.614 \\ \hline \hline
Ours           & \textbf{50.6}     & \textbf{81.5}  & \textbf{81.8}  & \textbf{0.596} & \textbf{0.682} \\\hline 
%\hline
%\multicolumn{6}{|c|}{(Old Non-Aligned) CMU-MOSEI Sentiment} \\ \hline \hline
%CTC~\citep{graves2006connectionist} + EF-LSTM  & 44.8     & 69.7  & 69.5  & 0.755 & 0.401 \\
%LF-LSTM        & 49.9     & 80.0  & 80.2  & 0.620 & 0.650 \\
%CTC + MCTN~\cite{pham2018found}     & 46.9     & 80.2  & 80.6  & 0.611 & 0.664 \\
%CTC + RAVEN~\cite{wang2018words}    & 48.9     & 76.2  & 77.0  & 0.681 & 0.576 \\ \hline \hline
%Ours           & \textbf{51.6}   & \textbf{81.8}  & \textbf{81.7}  & \textbf{0.586} & \textbf{0.697} \\ \hline
\end{tabular}
\end{center}
\end{table}

==> tables/shift_mosi.tex <==
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\begin{table}[t!]
\vspace{-5mm}
\caption{\small Results for multimodal sentiment analysis on CMU-MOSI with aligned and non-aligned multimodal sequences. For the models that cannot handle non-alignment, we perform  \emph{connectionist temporal classification} (CTC)~\citep{graves2006connectionist} on the input multimodal sequences, which pseudo-aligns different modalities before the multimodal training. ${}^h$ means higher is better and ${}^\ell$ means lower is better.}
\begin{center}
\fontsize{7}{10}\selectfont
%\centering
\setlength\tabcolsep{0.7pt}
\vspace{-2mm}
\begin{tabular}{|c||*{5}{K{0.77cm}}|}
\hline
Metric         & Acc$_7^h$  & Acc$_2^h$  & F1$^h$    & MAE$^l$   & Corr$^h$  \\ \hline \hline
\multicolumn{6}{|c|}{(Shifted) CMU-MOSI Sentiment} \\ \hline \hline
EF-LSTM  & 29.3     & 72.1  & 73.3  & 1.077 & 0.522 \\
LF-LSTM        & 34.5     & \bf{78.4}  & \bf{78.3}  & 0.993 & 0.618 \\
MCTN~\cite{pham2018found}     & 28.3     & 71.3  & 72.9  & 1.134 & 0.486 \\
RAVEN~\cite{wang2018words}    & 26.8     & 74.5  & 75.2  & 1.070 & 0.562 \\ \hline \hline
Ours           & \bf{37.0}     & 78.2  & 78.2  & \bf{0.940} & \bf{0.662}  \\ \hline 
%\hline
%\multicolumn{6}{|c|}{(Old Non-Aligned) CMU-MOSI Sentiment} \\ \hline \hline
%CTC~\citep{graves2006connectionist} + EF-LSTM  & 31.0     & 73.6  & 74.5  & 1.078 & 0.542 \\
%LF-LSTM        & 33.7     & 77.6  & 77.8  & 0.988 & 0.624 \\
%CTC + MCTN~\cite{pham2018found}     & 32.7     & 75.9  & 76.4  & 0.991 & 0.613 \\
%CTC + RAVEN~\cite{wang2018words}    & 31.7     & 72.7  & 73.1  & 1.076 & 0.544 \\ \hline \hline
%Ours           & \bf{38.9}     & \bf{83.7}  & \bf{83.5}  & \bf{0.865} & \bf{0.709} \\ \hline
\end{tabular}
\end{center}
\end{table}
